Effective Yet Ephemeral Propaganda Defense: There Needs to Be More than One-Shot Inoculation to Enhance Critical Thinking

In today's media landscape, propaganda distribution has a significant impact on society. It sows confusion, undermines democratic processes, and leads to increasingly difficult decision-making for news readers. We investigate the lasting effect on critical thinking and propaganda awareness on them when using a propaganda detection and contextualization tool. Building on inoculation theory, which suggests that preemptively exposing individuals to weakened forms of propaganda can improve their resilience against it, we integrate Kahneman's dual-system theory to measure the tools' impact on critical thinking. Through a two-phase online experiment, we measure the effect of several inoculation doses. Our findings show that while the tool increases critical thinking during its use, this increase vanishes without access to the tool. This indicates a single use of the tool does not create a lasting impact. We discuss the implications and propose possible approaches to improve the resilience against propaganda in the long-term.

==> sections/backup_06_discussion.tex <==
\section{Discussion}
%Idea: Contrast our work with theirs (related work)
Our work investigated whether and how an AI-based propaganda detection tool, designed with elements of inoculation, could foster CT of news readers.
Our approach integrated weakened forms of propaganda through three mechanisms detection of propaganda, explanations, and contextual information. Through these mechanisms, users are exposed to a weakened form of propaganda. The intention was to help users build a form of "mental immunity" against propaganda. However, our findings indicate that while there was an increase in CT when the tool was available, those benefits diminished once the tool was removed.

The core challenge appears to be that participants used the tool as a "crutch" rather than developing independent CT abilities. This dependency aligns with observations from recent research on LLM-based tools \cite{Bastani2024}, where overreliance also happened. This tool dependency suggests users defaulted to System 1 thinking instead of developing the deeper, more deliberate System 2 thinking processes essential for genuine CT.

When comparing our approach to successful inoculation implementations, particularly Roozenbeek et al.'s \cite{roozenbeek_psychological_2022} work, some key differences in implementation and mechanisms emerge. They used short videos, engaging stories, and visual elements to expose participants to weakened forms of propaganda techniques. In contrast our tool attempted to weaken existing propaganda through annotations. This suggest that our implementation of inoculation might be an issue and also that the mode of delivery plays a significant role.
Future work could explore incorporating storytelling elements, interactive exercises, or gamification to actively engage users in identifying propaganda techniques and to activate CT. Additionally, the mode of delivery could be enhanced by combining tool-based annotations with multimedia elements like short videos or interactive scenarios.



Our evaluation using Kahneman's framework extends beyond previous work, such as Russo et al.'s \cite{russo2023aide} conversational agent based study. 
While their work demonstrated benefits through story creation and evaluation, our approach revealed a crucial gap between assisted and independent CT. This measurement approach allowed us to quantify not just the immediate effects of AI assistance but also explain the cognitive mechanisms behind tool dependency.

Several other factors might also explain the limited retention of CT toward propaganda. First, the lack of emotional elements in our approach could play an important factor, as emotional engagement has been shown to play a crucial role in learning retention \cite{PHELPS2004198}. Second, as Maertens et al. \cite{maertens_long-term_2021} found in their work around long-term effectiveness of inoculation, a single exposure might be insufficient and repeated treatments "boosters" might be required.

Overall, our findings and related works show that while AI-based tools can effectively help with CT-heavy tasks, they struggle to create lasting improvements.


==> sections/backup_07_conclusion.tex <==
\subsection{Conclusion}
Our research examines the integration of a LLM-based tool with psychological frameworks, specifically investigating how automated propaganda detection and additional information complements traditional inoculation approaches. While our initial framing suggested a direct application of inoculation theory, our findings reveal a more nuanced relationship between technological assistance and inoculation principles.

In our experimental setup, participants were exposed to propaganda content alongside the tool's annotations and explanations, effectively creating a form of weakened exposure that aligns with inoculation theory principles. The tool's annotations served to highlight and explain propaganda techniques, potentially reducing their persuasive impact during the experiment. However, in practical applications, the tool functions differently - rather than pre-exposing users to weakened forms of propaganda, it provides real-time analysis and annotations that help "weaken" propaganda techniques as users encounter them naturally on websites.

We provide empirical evidence of how technological assistance and psychological frameworks interact, demonstrating that while our tool can enhance CT during its usage, creating lasting improvement requires a more sophisticated approach. This finding aligns with traditional inoculation theory, which typically involves carefully controlled exposure to weakened counterarguments - though our tool implements this weakening through real-time analysis rather than pre-planned exposure.

A key finding is the temporal nature of the tool's intervention. While participants have access to the tool, their CT and propaganda awareness increase significantly. However, without access to the tool, these increases vanish. This reveals that participants used the tool as a "crutch" and it did not assist in developing independent CT, suggesting that while the tool can effectively weaken propaganda in the moment, it may not create the lasting resistance that traditional inoculation approaches aim to achieve.

Our study raises important considerations about the content generated by LLM-based tools. While our tool aims to detect and explain propaganda and provides contextual information, it could also introduce its own biases or misinformation.

Potential limitations of our approach include our measurement methodology for CT, which relied on self-reported questionnaires. The study setup might not be optimally suited for testing inoculation effects, given the lack of participants' motivation to improve CT. Participants' motivation appeared more focused on completing the study rather than learning from it. Alternative approaches such as eye-tracking, neurological studies, or longitudinal observational studies could provide deeper insights into whether true inoculation effects occur. Additionally, the single-exposure treatment may not have been sufficient to establish new cognitive patterns or create the lasting resistance to persuasion that characterizes successful inoculation.

These insights suggest several promising directions for future research. To address engagement challenges, future research should explore interactive, emotional, and multimedia-based interventions to make the learning process more compelling. The issue of sustaining the learned skill could be tackled through spaced-repetition or booster interventions that combine the tool's real-time weakening capabilities with more traditional inoculation approaches.

The tool could be improved pedagogically to avoid being used as a crutch, perhaps by gradually reducing the level of annotation support while maintaining its ability to weaken propaganda techniques in real-time.

The challenge of combating propaganda requires a solution that can bridge the gap between immediate effect and long-term improvements in CT and propaganda awareness. One path forward could lie in creating a system that better balances real-time propaganda weakening with lasting skill development, focusing on strengthening users' ability to think critically and independently about the information they read, while carefully considering the potential risks of using AI-generated content.

